Biba's trick, with applications

We give another bit of evidence that forcing axioms provide proper framework for rigidity of quotient structures, by improving the OCA lifting theorem proved by the author in late 20th century and greatly simplifying its proof. In the assumptions of this theorem. We also extend the conclusion of author's 2004 lifting theorem from a lifting result for countably 3204-determined ideals to one for countably 80-determined ideals and weaken its assumptions.

==> olddefs.tex <==
% Definitions for LaTeX


\catcode`\@=11
\newdimen\ex@
\ex@.2326ex

\def\varprojlim{\mathop{\vtop{\halign{##\crcr
 \hfil\rm lim\hfil\crcr\noalign{\nointerlineskip}\leftarrowfill\crcr
 \noalign{\nointerlineskip\kern-\ex@}\crcr}}}}
\def\forces{\Vdash}
\def\p{{\mathcal P}}              % poset
\def\q{{\mathcal Q}}
\def\D{{\mathcal D}}
\def\N{\mathbb N}                        % Skup prirodnih brojeva
\def\R{{\mathbb R}}             % R, skup realnih brojeva
\def\Fin{{\rm Fin}}   % Konacne parcijalne funkcije
\def\I{{\mathcal I}} % Ideal 
\def\J{{\mathcal J}}
\def\U{{\mathcal U}} % Ultrafilter
\def\V{{\mathcal V}} % Ultrafilter
\def\W{{\mathcal W}} % Ultrafilter
\def\A{{\mathcal A}} 
\def\B{{\mathcal B}}   
\def\F{{\mathcal F}}
\def\OFin{\emptyset\times \Fin}
\def\FinO{\Fin\times\emptyset}
\def\FFin{\Fin\times\Fin}

\DeclareMathOperator{\dom}{dom}
\def\vert{\,:\,}
\def\Aut{\mbox{Aut}}
\def\X{{\mathcal X}}                       
\def\h{{\mathcal H}}
\def\Cal{\mathcal}
\def\<{\langle}
\def\>{\rangle}
\def\ssize{\scriptsize}
\def\rs{\restriction}
\def\text{\mbox}
\def\Exh{\mbox{Exh}}
\def\Nul{\mbox{Nul}}
\def\And{\quad\mbox{and}\quad}
\def\proof{\medbreak{\noindent\sc Proof}\quad}
\def\endproof{\medskip\qed}
\def\pmb{\bold}
\def\tsize{\normalsize}
%\def\theprop{Proposition}
\def\chGa{26} % gaps
\def\id{\mbox{id}}
\def\b{{\mathfrak b}}
\def\d{{\mathfrak d}}

\newtheorem{thm}{Theorem}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{theorem}[proposition]{Theorem}
\newtheorem{coro}[proposition]{Corollary}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{conjecture}[proposition]{Conjecture}
\newtheorem{conj}[proposition]{Conjecture}
\newtheorem{xtheorem}[proposition]{Theorem}
\newtheorem{question}[proposition]{Question}
\newtheorem{problem}[proposition]{Problem}
\newtheorem{claim}{Claim}
\newtheorem*{fact}{Fact}
\newtheorem*{subclaim}{Subclaim}


\theoremstyle{definition}
\newtheorem{definition}[proposition]{Definition}

\theoremstyle{remark}
\newtheorem{example}[proposition]{Example}
\newtheorem{remark}[proposition]{Remark}


\def\Nm#1{\|#1\|_\mu}
\def\TO#1{^{(#1)}}
\def\surj{\twoheadrightarrow}
\def\c{{\mathfrak c}}
\def\Fp#1#2{#1^{(#2)}}


\newcommand{\Iff}{\qquad\Leftrightarrow\qquad}

% version of 14 July  1997



\def\down#1{[#1]}
\def\id{\operatorname{id}}
\def\c{{\mathcal C}}
\def\twolo{\{0,1\}^{<\N}}
\def\twooo{\{0,1\}^{\omega_1}}
\def\twoloo{\{0,1\}^{<\omega_1}}
\def\oo{{}^\N\N}
\def\ooo{{}^\N(\oo)}
\def\kone{$\<\kappa,1\>$}
\def\kaplam{$\<\kappa,\lambda\>$}
\def\0{{\underline 0}}
\def\1{{\underline 1}}
\def\2{{\underline 2}}
\def\MM{{\frak M}}
\def\NMM{N^\MM}
\def\onetwo{\0,\1,\2}
\def\Ap{{\mathcal A}}
\def\LT{\vartriangleleft}
\def\sneqm{\sup\neq\max}
\def\init{\sqsubset}
\def\tini{\sqsubset}
%\def\niti{\sqsupset}
\def\h{{\mathcal H}}
\def\twoo{\{0,1\}^{\N}}
\def\pp{\p\p}
\def\pC{\p\c}
\def\i{i}
\def\imapsto{\buildrel \i\over \mapsto}

\DeclareMathOperator{\RB}{RB}
\DeclareMathOperator{\RK}{RK}
\DeclareMathOperator{\BA}{BA}
\DeclareMathOperator{\BE}{BE}
\DeclareMathOperator{\EM}{EM}
\DeclareMathOperator{\Bc}{Bc}
\DeclareMathOperator{\BC}{BC}

\def\Fa{{\mathcal F}}
\newcommand{\ucup}{\,\underline{\cup}\,}
\newcommand{\uDelta}{\,\underline{\Delta}\,}
\def\J{{\mathcal J}}
\def\lRB{\leq_{\RB}}
\def\lRK{\leq_{\RK}}
\def\lnRB{\lneq_{\RB}}
\def\lBE{\leq_{\BA}}
\def\lBa{\leq_{\BE}}
\def\lBo{\leq_{\BC}}
\def\lX{\leq_{\BE}^+}
\def\eBE{=_B}
\def\eBa{=_{\BA}}
\def\embeds{\hookrightarrow}
\def\lE{\leq_{\EM}}
\DeclareMathOperator{\add}{add}
\def\addN{\add(\Null)}
\def\abrsk{\<a,b\>\rs k=\<a',b'\>\rs k} 

\def\In#1{[n_#1,n_{#1+1})}
\def\even{{\text{even}}}
\def\Odd{{\text{odd}}}
\def\FIN{\operatorname{FIN}}
\def\Fin{\operatorname{Fin}}
\def\e{\varepsilon}
\def\G{{\mathcal G}}
\def\PSI#1{\Psi_{#1}}
\def\Sum{{\mathcal S}}
\def\Tr{\operatorname{Tr}}
\def\ab#1{\<a_{#1},b_{#1}\>}
\def\aB#1#2{\<a^{#1}_{#2},b^{#1}_{#2}\>}
\def\ij#1{\<i_{#1},j_{#1}\>}

\def\RLomega{[\Reals]^{<\omega}}

\def\finN{\fin\times \N}
\def\OFin{\emptyset\times \Fin}
\def\FinO{\Fin\times\emptyset}
\def\FFin{\Fin\times\Fin}
\def\FIN{$\Fin$}
\def\FINO{$\FinO$}
\def\OFIN{$\OFin$}

\def\Exh{\operatorname{Exh}}

\def\Pm{\{0,1\}^m}
\def\Pn{\{0,1\}^n}
\def\co{\complement}


\def\Zlog{{\mathcal Z_{\log}}}
\def\Zz{{\mathcal Z}_0}

\def\Di{{\mathcal Z}}
\def\EU{{\mathcal E\mathcal U}}
%\DeclareMathOperator{\Dom}{\supp}
\DeclareMathOperator{\atp}{at^+}
\DeclareMathOperator{\atm}{at^{--}}

\DeclareMathOperator{\branch}{br}
\DeclareMathOperator{\Ccont}{cont}
\def\Jbr{\J_{\branch}}
\newcommand{\Jcont}{\cJ_{\Ccont}}
\newcommand{\Jdec}{\cJ_{\mathrm{dec}}}
\newcommand{\Jcontnm}{\cJ_{\mathrm{cont*}}}
\newcommand{\Jsigma}{\cJ_\sigma}
\def\ZZ{{\mathcal Z}}
%\def\Jsig#1{\J_{\sigma}^{#1}}
%\def\Jc#1{\J_{\Ccont}^{#1}}

\def\Y{{\mathcal Y}}

\def\phi{\varphi}
\def\Np#1{\|#1\|_\phi}
\def\NP#1{\Biggl\|#1\Biggr\|_\phi}
\def\Npf#1{\|#1\|_{\phi_f}}
\def\Npm#1{\|#1\|_{\phi_\mu}}
\def\Npl#1{\|#1\|_{\phi_\lambda}}

\def\Pln{$\p(\twolo)/\Nwd$}
\def\NNN{$\N$}
\def\PNFin{$\p(\N)/\Fin$}
\def\PNFinO{$\p(\N^2)/\FinO$}

\def\FinFinO{$\Fin$ and $\FinO$}
\def\FINO{$\FinO$}
\def\f{{f}}

\def\BM{\operatorname{BM}}
\def\otp{\operatorname{otp}}
\def\C{{\mathcal C}}
\def\sco{{<_{\text{sc}}}}
\def\ci{\operatorname{ci}}
\def\lrk{\<k\>}


\def\Jdfin{\J_{d-\Fin}}
\def\Jtfin{\J_{2-\Fin}}
\def\bD{{\mathbb D}}
\def \cll#1{{\mathcal C}(#1)}
\def \clld#1{ \calL^d(#1)}
\def\Kd{\K^d}
\def\Kl{\K^l}
\def\Ialpha{\<\alpha\>}
\def\Igamma{\<\gamma\>}
\def\Idelta{\<\delta\>}
\def \cl{\operatorname{cl}}
\def\Bcl{\operatorname{cl}\TO d}
\def\TO#1{^{(#1)}}
\def\surj{\twoheadrightarrow}
\def\matbbD{{\mathbb D}}
\def\Rad{{\mathcal R}_\alpha^d}
\def\Rd{{\mathcal R}^d}
\def\pFin{\prod_n \p_n/\Fin}

\def\pNIepNJ{\p(\N)/\I\embeds \p(\N)/\J}
\def\pNI{\p(\N)/\I}
\def\Tukey{\equiv}
\def\pTukeyp{\p_1\Tukey\p_2}

\def\NNFin{\N^\N/\Fin}
\def\AUTpNI{\Aut(\p(\N)/\I)}

\font\BF=cmbx10 scaled \magstep 2
\font\RM=cmr10 scaled \magstep 2

\font\cyr=wncyr8
\font\cyrten=wncyr10
\font\itcyr=wncyi8


\def\Nwd{{\mathcal N}}
\def\Reals{{\mathbb R}}
\def\PartLo{$L^n_0(D)$}
\def\PartKo{$K^n_0$}


\newcommand{\IS}[2]{#2\index{#1!#2}}
\newcommand{\ISD}[2]{\index{#1!#2}}
\newcommand{\ID}[1]{}

\def\Na{\char'136{}}           
\renewcommand{\c}{{\mathfrak c}}
\newcommand{\II}[1]{#1\index{#1}}
\newcommand{\IIM}[2]{#2\index{#1@#2}}
\newcommand{\IC}[2]{#1\index{#1 #2}}
\newcommand{\SI}[1]{#1\index[symbol]{$#1$}}
\newcommand{\SD}[1]{\index[symbol]{$#1$}}
%\DeclareMathOperator{\log}{log}
\DeclareMathOperator{\AUT}{Aut}
\DeclareMathOperator{\cf}{cf}

\DeclareMathOperator{\DOM}{dom}
\DeclareMathOperator{\Stone}{Stone}
\DeclareMathOperator{\cpct}{{\mathcal K}}
\newcommand{\Basis}{{\mathcal  B}}
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\sfA}{{\sf A}}
\newcommand{\sfB}{{\sf B}}
\newcommand{\sfC}{{\sf C}}

\newcommand{\Null}{{\mathcal  N}}
\newcommand{\g}{{\mathfrak  g}}
\newcommand{\idK}{{\mathcal K}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\fr}{\frac}
\def\isom{\buildrel\sim\over =} 
\newcommand{\bfSigma}{{\boldsymbol\Sigma}}
\newcommand{\EE}{E}
\DeclareMathOperator{\RN}{RN}
\def\Pn{\p([1,n))}
\def\Pm{\p([1,m))}

\newcommand{\theDefinition}[1]{Definition \ref{#1}}
\newcommand{\theQuestion}[1]{Question \ref{#1}}
\newcommand{\theCoro}[1]{Corollary \ref{#1}}
\newcommand{\theprop}[1]{Proposition \ref{#1}}
%\newcommand{\thethm}[1]{Theorem \ref{#1}}
\newcommand{\theLemma}[1]{Lemma \ref{#1}}
\newcommand{\theExample}[1]{Example \ref{#1}}
\newcommand{\thettheorem}[1]{Theorem \ref{#1}}
\newcommand{\lasttheorem}[1]{Theorem \ref{#1}}
\newcommand{\lastlemma}[1]{Lemma \ref{#1}}
\newcommand{\lastprop}[1]{Proposition \ref{#1}}
\newcommand{\lastcoro}[1]{Corollary \ref{#1}}
\newcommand{\lastquestion}[1]{Question \ref{#1}}

\DeclareMathOperator{\ran}{range}
\DeclareMathOperator{\supp}{supp}

\newcommand{\case}[1]{\medbreak \noindent{\sc Case #1.}\quad}


\renewcommand{\proofname}{Proof}

% \begin{proof}[Proof of Claim]
% gives {\scshape Proof of Claim}. ...
% \begin{proof}[\it Proof]
% gives a proof with the proofname in italics

\renewenvironment{proof}[1][\proofname]{\par
\let\oldqedsymbol\qedsymbol             % Store \qedsymbol
  \normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep\hskip\parindent\scshape
    #1\@addpunct{.}]\ignorespaces
}{%
  \qed\endtrivlist
\global\let\qedsymbol\oldqedsymbol      % Restore it, if it had been changed
}

% Add the environment with no period after Proof
% For construction of the form
% Proof is by induction ...

\newenvironment{proofplain}[1][\proofname]{\par
\let\oldqedsymbol\qedsymbol             % Store \qedsymbol
  \normalfont
  \topsep6\p@\@plus6\p@ \trivlist
  \item[\hskip\labelsep\hskip\parindent\scshape
    #1] 
}{%
  \qed\endtrivlist
\global\let\qedsymbol\oldqedsymbol      % Restore it, if it had been changed
}


\newcommand{\glossaryentry}[2]{\item #1\dotfill #2\qquad}

\newcommand{\hinv}{h^{{-1}}}


%%% New 
\newcommand{\cP}{\mathcal P}
\newcommand{\calL}{\mathcal L}
\newcommand{\bbN}{\mathbb N}
\newcommand{\bbQ}{\mathbb Q}
\newcommand{\bbZ}{\mathbb Z}
\newcommand{\bbI}{\mathbb I}
\newcommand{\cI}{{\mathcal I}} % Ideal 
\newcommand{\cJ}{{\mathcal J}} % Ideal 
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cA}{\mathcal A}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cT}{\mathcal T}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}
\newcommand{\cW}{\mathcal W}

\newcommand{\cF}{\mathcal F}
\newcommand{\cG}{\mathcal G}
\newcommand{\calH}{\mathcal H}
\newcommand{\OOPS}{\marginpar{!!!!}}
\DeclareMathOperator{\OCAT}{OCA_T}
\DeclareMathOperator{\OCAinfty}{OCA_\infty}
\DeclareMathOperator{\OCAsharp}{OCA^\#}
\DeclareMathOperator{\NWD}{NWD}
\DeclareMathOperator{\NULL}{NULL}

\newcommand{\onezerosixeight}{1068}
\newcommand{\threetwozerofour}{3204}
\newcommand{\cS}{\mathcal S}
\newcommand{\bfc}{\mathbf c}

\newcommand{\bbP}{\mathbb P}
\newcommand{\calD}{{\mathcal D}}

\newcommand{\bbNN}{\bbN^\bbN}

%%%%%%%%%%%%%%%%%%%%%%%%%%added 2023

\newcommand{\cB}{\mathcal B}
\newcommand{\cstar}{$\mathrm{C}^*$}
\DeclareMathOperator{\MA}{MA}
\DeclareMathOperator{\MAsigma}{MA(\sigma-\text{linked})}
\DeclareMathOperator{\MAsc}{MA(\sigma-\text{centered})}
\DeclareMathOperator{\PFA}{PFA}
%\DeclareCommandCopy{\cof}{cof}

\newcommand{\cPN}{\cP(\bbN)}

\newcommand{\Xref}[1]{\marginpar{Reference #1}}
\newcommand{\WARNING}[1]{\marginpar{#1}}


\newcommand{\eqRK}{\sim_{\RK}}
\newcommand{\fb}{{\mathfrak b}}
\newcommand{\bbR}{{\mathbb R}}
\DeclareMathOperator{\Diff}{Diff}

\newcommand{\Sindex}[1]{\index[symbol]{#1}}
\newcommand{\INCLUDE}{\marginpar{\tt Include}}
\newcommand{\NOTE}[1]{\marginpar{\tt NOTE #1}}
\newcommand{\fc}{\mathfrak c}

\newcommand{\REMARK}[1]{\marginpar{\tt\small #1}}
\newcommand{\REFERENCE}{{\tt REFERENCE}}
\newcommand{\MOVE}{\REMARK{MOVE}}
\newcommand{\COMPUTE}{\REMARK{Compute}}


